Decentralized Control of Multi-Agent Systems Under Acyclic Spatio-Temporal Task Dependencies

We introduce a novel distributed sampled-data control method tailored for heterogeneous multi-agent systems under a global spatio-temporal task with acyclic dependencies. Specifically, we consider the global task as a conjunction of independent and collaborative tasks, defined over the absolute and relative states of agent pairs. Task dependencies in this form are then represented by a task graph, which we assume to be acyclic. From the given task graph, we provide an algorithmic approach to define a distributed sampled-data controller prioritizing the fulfilment of collaborative tasks as the primary objective, while fulfilling independent tasks unless they conflict with collaborative ones. Moreover, communication maintenance among collaborating agents is seamlessly enforced within the proposed control framework. A numerical simulation is provided to showcase the potential of our control framework.

==> content/collision_avoidance_section.tex <==
\begin{figure*}[h]
\centering
\begin{subfigure}{.3\textwidth}
  \centering
  \centerline{\includesvg[width=1.\columnwidth]{images/nu.svg}}
  \caption{}
  \label{fig: nu}
\end{subfigure}%
\begin{subfigure}{.3\textwidth}
  \centering
  \centerline{\includesvg[width=1.\columnwidth]{images/barriers.svg}}
  \caption{}
  \label{fig:barriers}
\end{subfigure}%
\begin{subfigure}{.3\textwidth}
  \centering
  \centerline{\includesvg[width=1.\columnwidth]{images/gamma.svg}}
  \caption{}
  \label{fig:gamma}
\end{subfigure}
\vspace{-0.8cm}\\
\begin{subfigure}{.3\textwidth}
  \centering
\centerline{\includesvg[width=0.8\columnwidth]{images/mas_ca.svg}}
  \caption{}
  \label{fig:mas_ca}
\end{subfigure}%
\begin{subfigure}{.3\textwidth}
  \centering
  \centerline{\includesvg[width=0.8\columnwidth]{images/prop_time.svg}}
  \caption{}
  \label{fig:prop_time}
\end{subfigure}%
\caption{ (a) Margin functions $\vec{\nu}^{\phi}_{ij}(\vec{e}_{ij}^k,t^k)$ for each barrier $b_{ij}^{\phi}(\vec{e}_{ij},t), b_{i}^{\phi}(\vec{x}_{i},t)$. (b) Barrier functions  $b_{ij}^{\phi}(\vec{e}^k_{ij},t^k),b_{i}^{\phi}(\vec{x}^k_{i},t^k)$ associated with tasks $\phi_{ij},\phi_i$. (c)  Control reduction factor $\gamma_i^k$. (d) MAS simulated over a time horizon of 50 sec. (e) Time required to propagate the value of $\gamma_i^k$ at each $k$ as per Alg. \ref{alg:control reduction alg}.}
\label{fig:mas sym big}
\end{figure*}
Collision avoidance and communication maintenance are equivalent to ensuring forward invariance of the sets $\mathcal{C}^a_{ij}=\{\vec{x} \in \mathbb{X} | \|\vec{p}_{ij}\| \geq r_i^a + r_j^a\},\; \forall (i,j)\in \mathcal{V}\times \mathcal{V}$ and $\mathcal{C}^c_{ij}=\{\vec{x} \in \mathbb{X} | \|\vec{p}_{ij}\| \leq r_c\}, \; \forall (i,j)\in \mathcal{E}_{\psi}$. Note that communication is only enforced among edges that are involved in collaborative tasks while collisions should be avoided among every agent. Since  $\mathcal{C}^c_{ij}$ corresponds to the level set of the predicate function $h^c_{ij}=r_c^2 - |\vec{p}_{ij}|^2$, which is concave, communication maintenance can be achieved by considering the STL tasks $\varphi_{ij}:= G_{[0,\infty]} h^c_{ij},\; \forall (i,j)\in \mathcal{G}_{\phi}$ such that the distributed controller \eqref{eq:new decentralised optimization with tasks} can be directly applied as explained in Sec. \ref{control} by including communication among the given tasks. On the other hand, $\mathcal{C}^a_{ij}$ is the level set of the sd-Lipschitz functions $b_{ij}^a(\vec{e}_{ij}) = ||\vec{p}_{ij}||^2- 4r_a^2$, which is concave and such that $\partial_{\vec{x}}b_{ij}^a \neq \vec{0} \, \forall \vec{x}\in \mathcal{C}_{ij}^a$. We then consider the sdCBF constraint $L_{\bar{f}}b^{a}_{ij}(\vec{e}_{ij}) + L_{\bar{g}}b^{a}_{ij}(\vec{e}_{ij})\vec{u}_{i} \geq -\zeta^{a}_{ij}(\vec{e}_{ij}^k)$ where we let $\zeta^{a}_{ij}(\vec{e}_{ij}^k) = \lambda_a b^a_{ij}(\vec{e}_{ij}) + \nu^a_{ij}(\vec{e}_{ij})$ as per \eqref{eq: local zeta}. Since safety is a critical aspect of the mission, we decide to compute a global $\nu^a_{ij}(\vec{e}_{ij}) = \nu^a_{ij}$ offline (so as to ensure the global minimum is found. See Remark \ref{remark on non convexity}) such that $\nu^a_{ij}\leq \bar{\nu}_{ij}^a(\vec{e}_{ij}) \, \forall \vec{x} \in \mathbb{X}$ as per \eqref{eq:local nu}. Note that this approach is different for $\nu_{ij}^{\phi}(\vec{e}_{ij},t)$ and $\nu_{i}^{\phi}(\vec{x}_{i},t)$ 
 as these are computed online at each instant $t^k$. A globally valid $\nu^a_{ij}$ is computed by solving the following non convex program \cite[Cor. 2]{breeden2021control}
\begin{equation}\label{eq:local nu avoidance} 
\begin{gathered}
\nu_{ij}^a = \min \bigl\{
L_{\bar{f}_i} b^a_{ij}(\vec{e}_{ij}) + L_{\bar{g}_i} b^a_{ij}(\vec{e}_{ij})\vec{u}_i + L_{\bar{f}_j} b^a_{ij}(\vec{e}_{ij}) + \\L_{\bar{g}_j} b^a_{ij}(\vec{e}_{ij})\vec{u}_j - \bigl(L_{\bar{f}_i} b^a_{ij}(\bar{\vec{e}}_{ij}) + L_{\bar{g}_i} b^a_{ij}(\bar{\vec{e}}_{ij})\vec{u}_i +\\ L_{\bar{f}_j} b^a_{ij}(\bar{\vec{e}}_{ij})  + L_{\bar{g}_j} b^a_{ij}(\bar{\vec{e}}_{ij})\vec{u}_j\bigr)  +\bigl(\lambda_a b_{ij}^a(\vec{e}_{ij}) -  \lambda_a b_{ij}^a(\bar{\vec{e}}_{ij})\bigr) \bigr\} \\
s.t :\; \vec{e}_{ij} \in \mathbb{X}_{ij}, \bar{\vec{e}}_{ij}\in \mathcal{R}_{ij}(\vec{e}_{ij},\delta t), \vec{u}_i\in \mathbb{U}_i,\vec{u}_j\in \mathbb{U}_j
\end{gathered}
\end{equation}
where $\mathcal{R}_{ij}(\vec{e}_{ij},\delta t)$ is the reachable set of relative states $\vec{e}_{ij}$. Note that this computation is only done once for each couple of dynamics. For instance, if the MAS is composed of agents with 3 different types of dynamics, then 6 different values of \eqref{eq:local nu avoidance} have to be computed, one for each couple of systems that can enter a collision. Then each agent employs the value of $\nu^a_{ij}$ corresponding to the agents it is trying to avoid. 
\begin{proposition}
Consider \eqref{eq:multi agent dynamics}, the functions $b^a_{ij}(\vec{e}_{ij}),\; \forall (i,j) \in \mathcal{V}\times \mathcal{V}$, the sensing set for agent $\mathcal{S}(i)$ defined as $\mathcal{S}(i) = \{ j \in \mathcal{V}| \|p_{ij}\| \leq r^s\}$ and let each agent be subject to a p.w.c control input  $\vec{u}_i(t)\in \mathcal{U}_i^{\delta t}$ such that $\vec{u}_i^k$ minimizes 

\begin{subequations}\label{eq:new decentralised optimization with tasks}
\begin{align}
& \min_{\substack{\vec{u}_i,s_i,s_{ij}\\ \text{as per \eqref{eq: leader constraint}-\eqref{eq: slack variables}}}} \vec{u}_i^T\vec{u}_i + c_i \, s_{i} + \sum_{j \in \mathcal{L}_{\psi}(i)} c_{ij}\,s_{ij} \\
&L_{\bar{f}_i} b^a_{ij}(\vec{e}^k_{ij}) + L_{\bar{g}_i} b^a_{ij}(\vec{e}^k_{ij})\vec{u}^k_i \geq \frac{1}{2}\zeta^a_{ij}(\vec{e}^k_{ij}) \; \forall j \in \mathcal{S}(i)
\end{align}
\end{subequations}
where $\zeta_{ij}(\vec{e}_{ij}^k) = \lambda_{a} b_{ij}^a(\vec{e}^k_{ij}) + \nu_{ij}^a$ and $\nu_{ij}^a$ is as per \eqref{eq:local nu avoidance}. Then $b_{ij}^a(\vec{e}_{ij})$ are sdCBF and if $\|\vec{p}_{ij}(t^0)\| \geq 2r_a$ holds at time $t^0$ then $\|\vec{p}_{ij}(t)\| \geq 2r_a\; \forall t\in \mathbb{R}_+$.
\end{proposition}
\begin{proof}
    Follows from Thm. \ref{main control theorem} and Lemma \ref{lemma local sample margin}.
\end{proof}

==> content/collsion_avoidance.tex <==

\section{Introducing collision avoidance and communication maintenance}\label{final design}
While objective 3) in problem \ref{main problem} is satisfied by direct application of the distributed control law \eqref{eq:new distributed optimization with tasks} we wish to ensure collision avoidance among agents while trying to satisfy the global task $\psi$ (objective 1)). Additionally, the connectivity maintenance condition $ \mathcal{G}_{\psi} \subseteq \mathcal{G}_{c}(t)$ (objective 2)) must be satisfied to fulfil $\psi_{col}$ itself such that communication is not a negotiable constraint along the edges $\mathcal{E}_{\psi}$. We employ the following classical locally Lipschitz (and thus sd-Lipschitz) function to encode the collision avoidance and communication constraints. 
\begin{subequations}
\begin{align}
&b_{ij}^a(\vec{e}_{ij}) = \vec{p}_{ij}^T\vec{p}_{ij} - (r_i^a + r_j^a)^2,  \label{eq:collsion avoidance sdcbf}\\
&b_{ij}^c(\vec{e}_{ij}) = (r^c)^2 - \vec{p}_{ij}^T\vec{p}_{ij} .\label{eq: communication sdcbf}
\end{align}
\end{subequations}
By letting $\zeta_{ij}^c(\vec{e}_{ij},t) = \lambda b^c_{ij} + \nu^c_{ij}$ and
$\zeta_{ij}^a(\vec{e}_{ij},t) = \lambda^a b^a_{ij} + \nu^a_{ij}$ we compute two constants $\nu^c_{ij}$ and $\nu^a_{ij}$ as
$$
\begin{aligned}
&  \nu_{ij}^c = \min_{\bar{\vec{e}}_{ij},\bar{\bar{\vec{e}}}_{ij},\bar{\vec{u}}_{i},\bar{\vec{u}}_j}  \\
& L_{f_i} b_{ij}^c(\bar{\vec{e}}_{ij}) - L_{f_i} b_{ij}^c(\bar{\bar{\vec{e}}}_{ij}) + 
(L_{g_i}b_{ij}^c(\bar{\vec{e}}_{ij})- L_{g_i}b_{ij}^c(\bar{\bar{\vec{e}}}_{ij}))\bar{\vec{u}}_i + \\
&L_{f_j} b_{ij}^c(\bar{\vec{e}}_{ij}) - L_{f_j} b_{ij}^c(\bar{\bar{\vec{e}}}_{ij}) +(L_{g_j}b_{ij}^c(\bar{\vec{e}}_{ij})- L_{g_j}b_{ij}^c(\bar{\bar{\vec{e}}}_{ij}))\bar{\vec{u}}_j +\\
& \lambda b_{ij}^c(\bar{\vec{e}}_{ij})-\lambda b_{ij}^c(\bar{\bar{\vec{e}}}_{ij})\\
&s.t \quad \bar{\vec{e}}_{ij}\in \mathbb{X}^c_{ij}, \bar{\bar{\vec{e}}}_{ij}\in  \mathcal{R}_{ij}(\bar{\vec{e}}_{ij},\delta t), \bar{\vec{u}}_i\in \mathbb{U}_i,\, \bar{\vec{u}}_j\in \mathbb{U}_j ,
\end{aligned}
$$
and
$$
\begin{aligned}
& \nu_{ij}^a = \min_{\bar{\vec{e}}_{ij},\bar{\bar{\vec{e}}}_{ij},\bar{\vec{u}}_{i},\bar{\vec{u}}_j}  \\
& L_{f_i} b_{ij}^a(\bar{\vec{e}}_{ij}) - L_{f_i} b_{ij}^a(\bar{\bar{\vec{e}}}_{ij}) + 
(L_{g_i}b_{ij}^a(\bar{\vec{e}}_{ij})- L_{g_i}b_{ij}^a(\bar{\bar{\vec{e}}}_{ij}))\bar{\vec{u}}_i + \\
&L_{f_j} b_{ij}^a(\bar{\vec{e}}_{ij}) - L_{f_j} b_{ij}^a(\bar{\bar{\vec{e}}}_{ij}) +(L_{g_j}b_{ij}^a(\bar{\vec{e}}_{ij})- L_{g_j}b_{ij}^a(\bar{\bar{\vec{e}}}_{ij}))\bar{\vec{u}}_j +\\
& \lambda b_{ij}^a(\bar{\vec{e}}_{ij})-\lambda b_{ij}^a(\bar{\bar{\vec{e}}}_{ij})\\
&s.t \quad \bar{\vec{e}}_{ij}\in \mathbb{X}^a_{ij}, \bar{\bar{\vec{e}}}_{ij}\in  \mathcal{R}_{ij}(\bar{\vec{e}}_{ij},\delta t), \bar{\vec{u}}_i\in \mathbb{U}_i,\, \bar{\vec{u}}_j\in \mathbb{U}_j ,
\end{aligned}
$$
where $X^c_{ij} = \{\vec{e}_{ij} | \|\vec{p}_{ij}\| \leq r^c \}$ and $X^a_{ij} = \{\vec{e}_{ij} | \|\vec{p}_{ij}\| \leq r^s \}$ represent the set of relative stated for which two agents can communicate with each other and sense each other respectively. We highlight that $\nu_{ij}^a$, $\nu_{ij}^c$ are not a function of the state or time such that they are computed offline. Morover, if we let $\nu_{ij}^a(\bar{\vec{e}}_{ij})$ and $\nu_{ij}^c(\bar{\vec{e}}_{ij})$ to be defined according to \eqref{eq:local nu} for $b_{ij}^a(\vec{e}_{ij})$ and $b_{ij}^c(\vec{e}_{ij})$ respectively, then by  \cite[Corl. 2]{breeden2021control} is holds that $\nu_{ij}^a \leq \nu_{ij}^a(\bar{\vec{e}}_{ij})$ and $\nu_{ij}^c \leq \nu_{ij}^c(\bar{\vec{e}}_{ij})$ where $\nu_{ij}^a(\bar{\vec{e}}_{ij})$, $\nu_{ij}^c(\bar{\vec{e}}_{ij})$.
\begin{proposition}
    Consider the time-varying communication graph $\mathcal{G}_c(t)$. If at each time instant $t_k$ it holds 
    \begin{equation}
    L_{f_i}b^{c}_{ij}(t^k) + L_{g_i}b^{c}_{ij}(t^k)\vec{u}^k_{i} \geq -\frac{1}{2}\zeta^{c}_{ij}(t^k)  \; \forall j\in \mathcal{N}_{c}(i) \label{eq: communication constraints}
    \end{equation}
    then $\mathcal{G}_{\psi} \subseteq \mathcal{G}_c(t^0) \Rightarrow \mathcal{G}_{\psi} \subseteq \mathcal{G}_c(t_0),  \; \forall t\in \mathbb{R}_+ $. If additionally, it holds at time $t^0$ that $\vec{b}_{ij}^a(\vec{e}_{ij}(t^0))\geq 0\;  \forall i,j\in \mathcal{V}$ and for each $t^k$ it holds 
    \begin{equation}
    L_{f_i}b^{a}_{ij}(t^k) + L_{g_i}b^{a}_{ij}(t^k)\vec{u}^k_{i} \geq -\frac{1}{2}\zeta^{a}_{ij}(t^k)  \; \forall j\in \mathcal{A}(i) \label{eq: collision constraints}
    \end{equation}
    where $\mathcal{A}(i) = \{j \in \mathcal{V} | \|\vec{p}_{ij}\| \leq r_s \}$, then all collisions among agents are avoided.
\end{proposition}
\begin{proof}
    By adding  \eqref{eq: communication constraints} or \eqref{eq: collision constraints} over an edge $(i,j)$, the sdCBF condition \eqref{eq: sdcbf condition} is obtained such that $b_{ij}^a(\vec{e}_{ij})$ and $b_{ij}^c(\vec{e}_{ij})$ are valid sdCBF. Lemma \ref{lemma local sample margin} then applies to prove the statement of the proposition. 
\end{proof}
\begin{remark}
    For the case of collision avoidance and connectivity maintenance, we let $\nu_{ij}^a$, $\nu_{ij}^c$ be computed offline instead of computing them online as we do for $\nu_{ij}^{\phi}$. The rationale behind this decision is that computing some $\nu_{ij}^a(\vec{e}_{ij},t)$ and $\nu_{ij}^c(\vec{e}_{ij},t)$ online (as we did for $\nu_{ij}^\phi(\vec{e}_{ij},t)$ in Sec. \ref{margin computation}) requires solving ulterior non-convex optimization problems for which finding global minimum cannot be guaranteed online (see Remark \ref{remark on non convexity}). Since, differently from the STL tasks, collision avoidance and communication maintenance are two critical tasks that guarantee the safety of the system, we decided to compute more conservative $\nu_{ij}^a(\vec{e}_{ij},t)$ and $\nu_{ij}^c(\vec{e}_{ij},t)$ offline such that strong minimization guarantees can be given (see. \cite[Sec IV]{breeden2021control} for a conservative analysis).
\end{remark}
With the purpose of solving objectives (1)-(3) of problem \ref{main problem} we decide to solve three optimization problems in parallel as per Table \ref{tab:parallel computation of optimal inputs} at each time instant $t^k$. When the primary controller A in Tab. \ref{tab:parallel computation of optimal inputs} is not feasible, then either backup solutions from B or C in Tab. \ref{tab:parallel computation of optimal inputs} are applied depending on if connectivity and collision avoidance (controller B) or only collision avoidance (controller C) can be ensured. Note that the infeasibility of controller A from some time instants $t^k$ does not necessarily imply that the global $\psi$ task will not be satisfied. Indeed for each collaborative task $\phi_{ij}$ with associated sdCBF $b_{ij}^{\phi}(\vec{e}_{ij},t)$, it is known that the level set $\mathcal{C}^{\phi}_{ij}(t)\, \forall (i,j)\in \mathcal{E}_{\psi}$ are asymptotically stable under controller A in Tab. \ref{tab:parallel computation of optimal inputs} (\cite[Remark 6]{cbfAron}) such that each $\phi_{ij}$ could eventually be satisfied or satisfied with some temporal delay.
% \begin{table}[]
%     \centering
%     \begin{tabular}{ccc}
%     \toprule
%     \toprule
%     \# &Objective &  Applied Controller at time $t^k$ \\
%     \midrule
%     A&(1),(2),(3)   & $\begin{gathered} \min_{\vec{u}_i\in \gamma_i^k \mathbb{U}_i} \vec{u}_i^T\vec{u}_i + c_is_{i} + \sum_{j \in \mathcal{L}_{\psi}(i)} c_{ij}s_{ij}\\ 
%         \vec{u}_i\in \mathbb{U}^{\phi}_i(t^k) \; \text{\eqref{eq: leader constraint}-\eqref{eq: slack variables}},
%         \vec{u}_i\in \mathbb{U}^{a}_i(t^k) \; \text{\eqref{eq: collision constraints}},\\
%         \vec{u}_i\in \mathbb{U}^{a}_i(t^k) \; \text{\eqref{eq: communication constraints}}\end{gathered}$ \\ 
%         \midrule
%     B&(1),(2)  & $\begin{gathered} \min_{\vec{u}_i\in \mathbb{U}_i} \vec{u}_i^T\vec{u}_i \\ 
%         \vec{u}_i\in \mathbb{U}^{a}_i(t^k) \; \text{\eqref{eq: collision constraints}}, \vec{u}_i\in \mathbb{U}^{c}_i(t^k) \; \text{\eqref{eq: communication constraints}}\end{gathered}$ \\ 
%        \midrule
%     C& (1)   & $\begin{gathered} \min_{\vec{u}_i\in \mathbb{U}_i} \vec{u}_i^T\vec{u}_i \\ 
%         \vec{u}_i\in \mathbb{U}^{a}_i(t^k) \; \text{\eqref{eq: collision constraints}}\end{gathered}$ \\ 
%         \bottomrule
%     \end{tabular}
%     \caption{Optimal inputs computed at each time at each time $t^k$}
%     \label{tab:parallel computation of optimal inputs}
% \end{table}


\begin{algorithm}[h]
\caption{Distributed control algorithm $i$}\label{alg:distributed control algorithm}
\begin{algorithmic}[1]
\STATE Initialise token sets $T_i$ as per Alg. \ref{alg:leadership propagation} (\#Seq)
\FOR{ $k\in \mathbb{N}_0$}
    \STATE Compute $\gamma_i^k$ over the network Alg. \ref{alg:control reduction alg} (\#Seq)
    \STATE Compute control inputs from A,B,C in Tab. \ref{tab:parallel computation of optimal inputs} and select the first feasible solution $\vec{u}_i^k$ in order of priority \eqref{eq:new distributed optimization with tasks} (\#Par)
\ENDFOR
\end{algorithmic}
\caption{Complete distributed control law.}
\end{algorithm}



